Distributed Multi-robot Online Sampling with Budget Constraints

In multi-robot informative path planning the problem is to find a route for each robot in a team to visit a set of locations that can provide the most useful data to reconstruct an unknown scalar field. In the budgeted version, each robot is subject to a travel budget limiting the distance it can travel. Our interest in this problem is motivated by applications in precision agriculture, where robots are used to collect measurements to estimate domain-relevant scalar parameters such as soil moisture or nitrates concentrations. In this paper, we propose an online, distributed multi-robot sampling algorithm based on Monte Carlo Tree Search (MCTS) where each robot iteratively selects the next sampling location through communication with other robots and considering its remaining budget. We evaluate our proposed method for varying team sizes and in different environments, and we compare our solution with four different baseline methods. Our experiments show that our solution outperforms the baselines when the budget is tight by collecting measurements leading to smaller reconstruction errors.

==> sections/relateworkbackup.tex <==
\section{Related Work}
\label{relwork}
In multi-robot sampling and monitoring, sectioning and Voronoi partitioning are common approaches; however, these methods assume that the distribution model of the environment is known beforehand, which is not practical in a real environment with an unknown model~\cite{suryan2022efficient}. Therefore, online sampling and dynamic Voronoi partitioning are needed. In~\cite{kemna2017multi}, they proposed the dynamic Voronoi approach, whereby robots repeatedly compute Voronoi partitions and each robot performs sampling within their partition. Although it seems that this method divides the exploration task efficiently between robots, in a noisy unknown environment, they should spend more time to find the optimal partition and sample their own partition, which in our case, with a tight budget, is not practical.

In~\cite{thayer2018multi}, they studied multirobot routing in a vineyard formulated as a team Orienteering problem. As part of the Orienteering problem, an agent is required to traverse a graph in which each vertex has a predetermined reward and each edge has a defined cost. A path should be computed that maximizes the sum of rewards while ensuring that the sum of the costs of traversing edges does not exceed the budget assigned in advance. Team Orienteering Problem (TOP) is a version of OP in which a team of robots works together to collect rewards. Their study examined three methods. The first method involved splitting the graph into $M$ disjoint segments and assigning one agent to each segment. It is important to note that sectioning has one major disadvantage: if one robot malfunctions, the section will not be explored. Next, robots were sent sequentially for the purpose of collecting rewards, zeroing the rewards that have been collected by each of them. Thirdly, they considered the centralized parallel Greedy Partial Row Heuristic algorithm (GPR), in which the most efficient path for each robot is stored in a list to be assigned to each robot later. 


Recently, MCTS has gained a great deal of attention for multi-robot IPP. In~\cite{jang2021fully, best2019dec}, they conducted research on combining Gaussian process and MCTS to solve the the environmental modeling estimation. In~\cite{manjanna2021scalable}, they proposed a decentralized approach using a policy gradient based approach for the application of multi-robot environment monitoring and sampling. To encourage robots to move far from coworkers, robot $k$ has a reward function dependent on its distance from them. Furthermore, they have considered a communication range between robots to exchange locations and the history of previous locations with co-working robots. In~\cite{pan2022marlas}, a decentralized adaptive sampling method for multi-agent scenarios was proposed which was robust to the failure of robots and communication failures. In order to estimate the optimal policy, they used deep neural networks and policy gradient methods. Their works, however, did not explicitly incorporate budgetary considerations. 

In~\cite{boothdistributed}, they considered the problem of reconstructing spatial field using multirobot, Gaussian process and MCTS. As part of their work, robots communicate with one another and send their current location and observations to other robots. In our work, which is a continuation of this work, we will estimate the next location that might be visited by other robots (within estimation range) so that it can be eliminated from the list of next candidates for the current robot. Also, we consider that all robots can exchange their past experiences (visited locations). We do not want two robots visiting the same place at the same time.

Various approaches can be used to solve reinforcement learning problems in which constraints must be met. Lagrangian methods include constraints in the loss function, while another method restricts the action space directly before choosing the next action. Our method uses a reward shaping technique. In~\cite{ge2019safe}, they used the Lagrange multiplier method to combine the cost function with constraint in order to determine the next action and analyze constrained Q-learning for robot path planning in a grid environment to avoid the trap. To demonstrate that their proposed method was able to find the better path, resulting in better return values in each episode, they compared their method with baseline SARSA and Q-learning. Using this method, there is no guarantee that the agent will satisfy the constraints at all points, which may result in undesirable behavior. In~\cite{kalweit2020deep}, they proposed an off-policy reinforcement learning framework in which the action space is limited in the Q-update in order to learn the optimal Q-function for the constrained MDP. First, the safe set of states is calculated for all constraints, then the deep Q-learning algorithm is applied. In on-policy learning, the $Q(s,a)$ function is learned from the actions the agent takes using its current policy $\pi(a|s)$. In off-policy learning, the $Q(s,a)$ function is acquired by taking different actions (for example, random actions). 
